Validation of Abstract Side-Channel Models for Computer Architectures

Observational models make tractable the analysis of information flow properties by providing an abstraction of side channels. We introduce a methodology and a tool, Scam-V, to validate observational models for modern computer architectures. We combine symbolic execution, relational analysis, and different program generation techniques to generate experiments and validate the models. An experiment consists of a randomly generated program together with two inputs that are observationally equivalent according to the model under the test. Validation is done by checking indistinguishability of the two inputs on real hardware by executing the program and analyzing the side channel. We have evaluated our framework by validating models that abstract the data-cache side channel of a Raspberry Pi 3 board with a processor implementing the ARMv8-A architecture. Our results show that Scam-V can identify bugs in the implementation of the models and generate test programs which invalidate the models due to hidden microarchitectural behavior.

==> design.tex <==
\section{Design}
\todo{1.5 pages Roberto + Andreas, Merge into intro}
\label{sec:design}

\begin{figure}[t]
  \includegraphics[width=0.9\linewidth]{architecture2.pdf}
  \caption{Validation framework architecture}
  \label{fig:arch}
\end{figure}

% Tool architecture (weakest relation syntheses)
We describe the basic ideas of our validation framework.
At a high level,  \tool\ generates random binaries and attempts to construct different initial states that lead to equivalent observations at the level of the model, but distinguishable on the real hardware. In essence, finding such counterexamples implies that the
model of the side channel is not precise enough, and leads to a potential
vulnerability. Figure~\ref{fig:arch} illustrates the main workflow of \tool.


The first step of our workflow involves 
generation of binaries for a given architecture.
We describe in Section~\ref{sec:program-generation} the different approaches 
that we currently use to generate programs.

\todo{This can be  purely random or based on some heuristics, 
like {model counting}~\cite{10.1007/978-3-642-01929-6_10} or {feed-back 
directed}~\cite{Pacheco:2007:FRT:1248820.1248841}, to generate more 
meaningful binaries.
RG: in related work
}

The second step  transforms the binary into BIR~\cite{Lindner2019},
via a process called \emph{lifting}~\cite{bir:lifter}. This
transformation reuses formal models of the ISAs, which have been used
in various projects to verify functional correctness of
binaries~\cite{sel4,cackeml}, and generates a proof that certifies
correctness of the translation.
In order to validate a given observational model, we extended this
process to inline observation statements into the resulting BIR
program. These observations represent the observational power of the side channel.

Then, we synthesize the weakest relation on
program states that guarantees observational equivalence, as described
in Section~\ref{sec:relation}. This relation is used to drive the
generation of \emph{test cases} -- states that can be used as inputs
to the program\todo{ -- in an approach based on SMT solving. RG: Not
  here}, as detailed in Section~\ref{sec:test-generation}.

Finally, we  run the generated binary with different test cases on the real hardware, and % (Test on processor)
we measure the side channel.
Since the chosen test cases satisfy the synthesized relation,
soundness of the model would imply that they cannot be distinguished
on the real hardware either. Otherwise, we have found a counterexample
to soundness that is reported to the user. 

If we did not find a counterexample, the framework can either generate
more test cases for the same program 
or restart the process for a new binary.

% HOL4 (including the models)

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> weakest-relation.tex <==
\newcommand{\symstate}{\sigma}
\newcommand{\initialsymbol}[1]{\mathbf{#1}}
\newcommand{\symexp}[1]{\mathbf{#1}}
\newcommand{\sympc}[1]{i_{#1}}
\newcommand{\sympath}[1]{\symexp{p}_{#1}}
\newcommand{\symmap}[1]{\symexp{M}_{#1}}
\newcommand{\symlist}[1]{\symexp{l}_{#1}}
\newcommand{\mapping}[2]{{#1} \rightarrow {#2}}

\newcommand{\birhalt}{$HALT$}
\newcommand{\birjmp}[1]{$JMP\ #1$}
\newcommand{\bircjmp}[3]{$CJMP\ #1\ #2\ #3$}
\newcommand{\birobs}[2]{$OBS\ #1\ #2$}

\newcommand{\cons}{\circ}

\section{Synthesis of Weakest relation}
\todo{Roberto: review}
Synthesis of the weakest relation is based on standard symbolic
execution techniques.
In the following we  use $\initialsymbol{X}$ to range over symbols,
and $\symexp{c}$, $\symexp{e}$, and
$\symexp{p}$ to range over symbolic expressions.
A symbolic state $\symstate$ consists of a concrete program counter
$\sympc{\symstate}$,
a path condition $\sympath{\symstate}$,
and a mapping $\symmap{\symstate}$ from variables to symbolic
expressions.
We write $e(\symstate) = \symexp{e}$ for the
symbolic evaluation of the expression $e$ in $\symstate$,  
and $\symexp{e}(s)$ for 
the value obtained by substituting the symbols of the symbolic
expression $\symexp{e}$ with the variable values in $s$.


\todo{RG remove this part}
The program counter of the initial state points to the
entry point of the program and the mapping simply maps each variable
$X$ to the corresponding symbolic value $\initialsymbol{X}$.
The symbolic execution iteratively pops a state $\symstate$ from the list
of pending states, executes the internal statements of the block
pointed by $\sympc{\symstate}$, updates 
$\symmap{\symstate}$ by symbolically evaluating the expressions of
assignments, and executes the control flow
instruction.
In case of \birhalt\ it adds the resulting state to the list of terminating states;
in case of \birjmp{l_1}\ it sets $\sympc{\symstate} = l_1$ and  
adds the resulting state to the list of pending states;
in case of \bircjmp{c}{l_1}{l_2} it evaluates $\symexp{c} =
c(\symstate)$ and adds states $\symstate_1, \symstate_2$ to the list of pending
states, where 
$\symmap{\sigma_i} = \symmap{\sigma}$, $\sympc{\sigma_i}=l_i$, 
$\sympath{\symstate_i} = \sympath{\symstate} \land \symexp{c}$,
$\sympath{\symstate_2} = \sympath{\symstate} \land \neg \symexp{c}$.


Symbolic execution of the example produces two terminating states
$\symstate_1$ and $\symstate_2$, which correspond to the two branches.
For the first branch $\sympath{\symstate_1} = \initialsymbol{Z}$ and
$\symmap{\symstate_1} = 
\{
\mapping{X_1}{\initialsymbol{X}_1+8},
\mapping{X_2}{LOAD(\initialsymbol{M}, \initialsymbol{X}_1)},
\}
$ (we omit the variables that are not updated).
For the second branch 
$\sympath{\symstate_2} = \neg \initialsymbol{Z}$ and
$\symmap{\symstate_2} = 
\{
\mapping{X_1}{\initialsymbol{X}_2 * \initialsymbol{X}_3 + 8},
\mapping{X_2}{LOAD(\initialsymbol{M}, \initialsymbol{X}_2 * \initialsymbol{X}_3)}
\}
$.




Standard symbolic execution is extended to handle observations:
The state is extended with a symbolic list $\symlist{\symstate}$;
The execution of \birobs{c}{\vec e} in $\symstate$
appends the pair $(\symexp{c}, \vec
{\symexp{e}})$ to $\symlist{\symstate}$ ,
where $\symexp{c} = c(\symstate)$ and $\vec {\symexp{e}}[i] = \vec {e}[i](\symstate)$.
%
For instance, in the case of observational model (1b) the
lists of the terminating states are:
\[
  \begin{array}{l l lll}
    \symlist{\symstate_1} & = [(T, [1,\initialsymbol{Z}]), & (T, [3])]\\
    \symlist{\symstate_2} & = [(T, [1,\neg \initialsymbol{Z}]), &
                            (T, [2, (\initialsymbol{X}_2 >
                            2^{16} \vee \initialsymbol{X}_3 >
                                                                  2^{16})]), &
                            (T, [3])]\\
  \end{array}
\]
and for the observational model (2b) we have:
\[
  \begin{array}{ll}
    \symlist{\symstate_1} & = [(\initialsymbol{X}_1 \& lines > 0,  [\initialsymbol{X}_1 \& tag])]\\
    \symlist{\symstate_1} & = [
                            ((\initialsymbol{X}_2 *\initialsymbol{X}_3) \& lines > 0,
                            [(\initialsymbol{X}_2 * \initialsymbol{X}_3) \& tag])]
  \end{array}
\]

Let $\Sigma$ be the set of terminating states produced by the symbolic
execution, $s$ be a concrete state, and 
$\symstate \in \Sigma$
be such that $\sympath{\symstate}(s)$ holds, 
the final value of variable $X$ when the program is executed starting
in $s$
is $\symmap{\symstate}(X)(s)$.
Moreover, let
$\symlist{\symstate} = [(\symexp{c_1, {\vec {\symexp{e}}_1}}) \dots
(\symexp{c_n, {\vec {\symexp{e}}_n}})]$
then the produced observations are $(\symexp{c_1, {\vec {\symexp{e}}_1}})(s)
\cons \dots \cons (\symexp{c_n, {\vec {\symexp{e}}_n}})(s)$,
where $(\symexp{c_1, {\vec {\symexp{e}}_1}})(s) = [{\vec
  {\symexp{e}}}_1(s)]$ if $\symexp{c}(s)$ otherwise $[]$. 

Therefore, the observation equivalent relation can be computed by
ensuring that for every possible pair of execution paths the resulting
observation lists are equivalent. Formally $s_1 \sim s_2$ is
\[
\bigwedge_{(\symstate_1, \symstate_2) \in \Sigma \times \Sigma}
(\sympath{\symstate_1}(s_1) \land \sympath{\symstate_2}(s_2) \Rightarrow
(\symlist{\symstate_1}, s_1) \sim (\symlist{\symstate_2}, s_2))
\]
where the equivalence of the symbolic observation list can be computed as
\[
  \begin{array}{lrl}
    \multicolumn{3}{l}
{    ((\symexp{c_1, {\vec {\symexp{e}}_1}}) \cons
    \symexp{l_1}, s_1) \sim
    ((\symexp{c_2, {\vec {\symexp{e}}_2}}) \cons
    \symexp{l_2}, s_2) \triangleq}
    \\
    \mbox{ }
    &
      \symexp{c_1}(s_1) \land \symexp{c_2}(s_2)
    &
      \Rightarrow
    \vec{\symexp{e_1}}(s_1) = \vec{\symexp{e_2}}(s_2) \land
    (\symexp{l_1}, s_1) \sim (\symexp{l_2}, s_2)\\
    \land
    &
      \neg \symexp{c_1}(s_1)
    &
      \Rightarrow
    (\symexp{l_1}, s_1) \sim ((\symexp{c_2, {\vec
    {\symexp{e}}_2}}) \cons \symexp{l_2}, s_2)\\
    \land
    &
      \neg \symexp{c_2}(s_2)
    &
      \Rightarrow
    ((\symexp{c_1, {\vec
    {\symexp{e}}_1}}) \cons \symexp{l_1}, s_1) \sim
    (\symexp{l_2}, s_2)\\[10pt]
    %
\multicolumn{3}{l}
{    ((\symexp{c_1, {\vec {\symexp{e}}_1}}) \cons
    \symexp{l_1}, s_1) \sim
    (([], s_2) \triangleq
    \neg \symexp{c_1}(s_1) \land (\symexp{l_1}, s_1) \sim ([], s_2)
    }\\[10pt]
    % %
\multicolumn{3}{l}
{    ([], s_1) \sim
    ((\symexp{c_2, {\vec {\symexp{e}}_2}}) \cons
    \symexp{l_2}, s_2) \triangleq
    \neg \symexp{c_2}(s_2) \land ([], s_1) \sim (\symexp{l_1}, s_2)}
    \\[10pt]
    %
\multicolumn{3}{l}{
    ([], s_1) \sim
    ([], s_2) \triangleq T}
  \end{array}
  \]

For the purpose of generating input test case we can syntetize a
smaller relation, since we do not need to handle both $(\symstate_1,
\symstate_2)$ and
$(\symstate_2, \symstate_1)$. Therefore, the syntetized relation is
\[
  \bigwedge_{
    \begin{array}{c}
      i \in \{1 \dots |\Sigma|\}\\
      j \in \{i \dots |\Sigma|\}\\
      \symstate_1 = \Sigma[i] \\ \symstate_2 =  \Sigma[j]
    \end{array}
  }
(\sympath{\symstate_1}(s_1) \land \sympath{\symstate_2}(s_2) \Rightarrow
(\symlist{\symstate_1}, s_1) \sim (\symlist{\symstate_2}, s_2))
\]


\todo{Optimization for non symmetric i.e. j >= i}
Therefore, for in the case of the observational model (o2.b) we have
that the syntetized relation is
\[
  \begin{array}{l}
    \initialsymbol{Z} \land \initialsymbol{Z'} \Rightarrow
    ((\initialsymbol{X}_1 \& lines > 0) \land
    (\initialsymbol{X'}_1 \& lines > 0)
    \Rightarrow
    (\initialsymbol{X}_1 \& tag = \initialsymbol{X'}_1 \& tag) 
    ) \\
    \land 
    \initialsymbol{Z} \land \initialsymbol{Z'} \Rightarrow
    (\neg (\initialsymbol{X}_1 \& lines > 0)
    \Rightarrow
    \neg (\initialsymbol{X}_2 \& lines > 0)
    ) \\
    \land 
    \initialsymbol{Z} \land \initialsymbol{Z'} \Rightarrow
    (\neg (\initialsymbol{X}_2 \& lines > 0)
    \Rightarrow
    \neg (\initialsymbol{X}_1 \& lines > 0)
    ) \\
    %
    \initialsymbol{Z} \land \neg \initialsymbol{Z'} \Rightarrow
    ((\initialsymbol{X}_1 \& lines > 0) \land
    ((\initialsymbol{X'}_2 * \initialsymbol{X'}_3) \& lines > 0)
    \Rightarrow
    (\initialsymbol{X}_1 \& tag = (\initialsymbol{X'}_2 * \initialsymbol{X'}_3) \& tag) 
    ) \\
    \land 
    \initialsymbol{Z} \land \neg \initialsymbol{Z'} \Rightarrow
    (\neg (\initialsymbol{X}_1 \& lines > 0)
    \Rightarrow
    \neg ((\initialsymbol{X'}_2 * \initialsymbol{X'}_3) \& lines > 0)
    ) \\
    \land 
    \initialsymbol{Z} \land \neg \initialsymbol{Z'} \Rightarrow
    (\neg ((\initialsymbol{X'}_2 * \initialsymbol{X'}_3) \& lines > 0)
    \Rightarrow
    \neg (\initialsymbol{X}_1 \& lines > 0)
    ) \\
    %
    \neg \initialsymbol{Z} \land \neg \initialsymbol{Z'} \Rightarrow
    (((\initialsymbol{X}_2 * \initialsymbol{X}_3) \& lines > 0) \land
    ((\initialsymbol{X'}_2 * \initialsymbol{X'}_3) \& lines > 0)
    \Rightarrow
    ((\initialsymbol{X}_2 * \initialsymbol{X}_3) \& tag = (\initialsymbol{X'}_2 * \initialsymbol{X'}_3) \& tag) 
    ) \\
    \land 
    \neg \initialsymbol{Z} \land \neg \initialsymbol{Z'} \Rightarrow
    (\neg ((\initialsymbol{X}_2 * \initialsymbol{X}_3) \& lines > 0)
    \Rightarrow
    \neg ((\initialsymbol{X'}_2 * \initialsymbol{X'}_3) \& lines > 0)
    ) \\
    \land 
    \neg \initialsymbol{Z} \land \neg \initialsymbol{Z'} \Rightarrow
    (\neg ((\initialsymbol{X'}_2 * \initialsymbol{X'}_3) \& lines > 0)
    \Rightarrow
    \neg ((\initialsymbol{X}_2 * \initialsymbol{X}_3) \& lines > 0)
    )
\end{array}
\]

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

